ATOM: An Efficient Topology Adaptive Algorithm for Minor Embedding in Quantum Computing

Quantum annealing (QA) has emerged as a powerful technique to solve optimization problems by taking advantages of quantum physics. In QA process, a bottleneck that may prevent QA to scale up is minor embedding step in which we embed optimization problems represented by a graph, called logical graph, to Quantum Processing Unit (QPU) topology of quantum computers, represented by another graph, call hardware graph. Existing methods for minor embedding require a significant amount of running time in a large-scale graph embedding. To overcome this problem, in this paper, we introduce a novel notion of adaptive topology which is an expandable subgraph of the hardware graph. From that, we develop a minor embedding algorithm, namely Adaptive TOpology eMbedding (ATOM). ATOM iteratively selects a node from the logical graph, and embeds it to the adaptive topology of the hardware graph. Our experimental results show that ATOM is able to provide a feasible embedding in much smaller running time than that of the state-of-the-art without compromising the quality of resulting embedding.

==> draft.tex <==
Based on the expandable characteristic of current QPU topologies, in this paper, we propose a novel heuristic method which can:
\begin{itemize}
    \item guarantee to return a feasible solution after at most $2\times |V(P)|$ iterations.
    \item achieve running time that outperforms both OCTs\cite{Goodrich2018} - the-state-of-the-art method for general topology of logical graphs and DWave's commercial method based on \cite{Cai2014} - the-state-of-the-art heuristic method for minor embedding in case of large sparse graphs.
    \item manipulate the hardware's size such that the size is increased along with the cardinity of the embedding.
\end{itemize}

Based on the grid structure of the QPU topology we mentioned in the last section, we realize that the hardware graph representing topologies $T(n,m,c)$ can be expandable. It means that we can construct a hardware graph with larger topology $T(n',m',c)$ from former hardware graph with smaller one $T(n,m,c)$ ($n \leq n'$ or $m \leq m'$) without violating any conditions of current embedding in the former hardware graph.

We can only finish a \emph{turn} of embedding, and move to the next \emph{turn} if the state variable $dead\_end$ get a value of \textit{False}. If not, we keep running at the current \emph{turn} until $dead\_end$ turns \textit{False}.

proof for lemma 1.
It is obvious that $\phi'$ is a feasible embedding of a graph $G$ with $V(G) = A \cup \{\Bar{v}\}$ and $E(G) = \{(\Bar{v}, v)|\forall v \in A\}$. At the end of the $(i)^{th}$ turn, we can obtain $\phi_{i}$ such that $\phi_{i}(v) = \phi_{i-1}(v) \cup \phi'(v)$ for $\forall v \in P$ that is a feasible embedding of $P[S_{i}]$.

proof for lemma 2.
We can see that after expanding, in the hardware graph $H$, there are rows including all column semi unit cells and empty unit cells, and columns including all row semi unit cells and empty unit cells. In addition, there always exists at least one clean path from nodes in a column semi unit cell to all other unit cell in the same row, and from nodes in a row semi unit cell to all other unit cell in the same column. It implies that there exists at least one clean path from nodes in semi unit cells to all other semi unit cells and empty unit cells. On the other hand, based on the rule of assignment, every chains $\phi(v) \neq \emptyset$ with $v \in V_P$ include at least one node in semi unit cells. As a result, there exists a free node that is able to connect to every chains $\phi(v)$ with $v \in A \subseteq V_P$ by clean paths.

As a result, it opens opportunities to solve notorious optimization problems which have not been effectively solved by traditional computers. Two common paradigms in quantum computing are gate-based model and Quantum Annealing (QA). Gate-based model is one type of quantum computer which obtains the output by measurement after transforming the input through a sequence of quantum gates. Although gate-based model has shown its ability to produce approximate solutions for optimization problems \cite{Farhi2014}, its fundamental limitation is that the number of quantum bits (qubits) in current technology is very limited, making it difficult to use quantum computing for large-scale inputs.


We describe QA process through the concept of Hamiltonian function. In a quantum system, a Hamiltonian is a function that maps eigenstates of the quantum system to energies. QA models such as DWave's quantum computers \cite{DWave_product} define the Hamiltonian of the quantum system as a combination of a initial and final Hamiltonians. The system begins with the lowest energy state (i.e. ground state) of initial Hamiltonian. It keeps the lowest energy throughout the quantum annealing process and ends up with the ground state of the final Hamiltonian. While this strategy chooses initial Hamiltonian in a way that the ground state of the initial Hamiltonian can be set up easily at the beginning, it needs to design the final Hamiltonian such that the ground state of the final Hamiltonian indicates the optimal solution for the desired problem.

QA evolves the ground state of a Hamiltonian to that of final Hamiltonian \cite{Yarkoni2022} through several stages shown in Figure 1. First, we convert the given optimization problem to a quadratic unconstrained binary optimization (QUBO) form. We then construct a graph called logical graph with nodes and edges representing variables and dependencies of the quadratic operators in the QUBO form respectively. Next, we map the resulting logical graph on a special graph, named hardware graph, which represents qubits and qubits' interactions in the Quantum Processing Unit (QPU) and finally, run annealing process repeadly to find the solution with the lowest energy. Notice that the topology of the hardware graph or its induced sub-graphs  may not be identical to that of the logical graph. Therefore, there is a need to find a mapping from the logical graph to the hardware graph such that every connections in the logical graph are preserved. That is called \textbf{minor embedding problem}.

We elaborate the assignment as follows. For each clean shortest path $Z_{\Bar{u} v}$ with $v \in A$, we splits the \emph{clean path} into two parts: the first part assigned to the chain $\phi(\Bar{v})$ and the second one assigned to the chain of $\phi(v)$. We can realize that free nodes which belongs to more than one clean shortest path from $\phi(\Bar{v})$ to $\phi(v)$ with $v \in A$ only can be assigned to the chain $\phi(\Bar{v})$. Therefore, we select the splitting index $i_v$ of the path $Z_{\Bar{u} v}$ as the biggest index such that $z_{i_v}$ belonging to more than one path. We also extend the splitting index $i_v$ by a range of $\delta$ which depends on the degrees of $\Bar{v}$ and $v$ in $P$. Then, we assign all free nodes in clean paths $Z_{\Bar{u} v}$ with $v \in A$ to the set of chains $\phi'$ depending on the splitting points $i_v$.

==> relatedworks.tex <==
%\tk{plan how you organize the literature in different paragraphs. Do you organize them by the type of problem they solve? by chronology? currently the organization is chaotic}


%\hoang{Actually, I plan to organize them by their direction and chronology. There are 2 main directions for embedding a graph P in hardware H: 1,embed complete graph $K_{|V_P|}$ and try to reduce to P. (call it top-down approach). 2, build embedding of P node-by-node (call it bottom-up approach). My organization in the literature is 1, review top-down approach by chronology(first 2 graphs). 2, show some limitation of top-down which can be solved by bottom-up and switch to review bottom-up approach by chronology(third graph). 3, show limitation of both in specific cases and from that, propose what we gonna do(forth graph) - work as a transition to next part in our paper}

%\mt{This related work is too lengthy. We can remove this section. We can blend a few key related work (each just has a line or so) in the Introduction.}

Two main approaches to do minor embedding are top-down and bottom-up. Choi introduced the minor embedding problem in QA \cite{Choi2008} and then, developed the first top-down solution for this problem \cite{Choi2011}. In his solution, Choi proposed an optimal edge-length bounded layout to embed complete graphs, called TRIAD. Choi showed that every complete graph can be embedded into a Chimera graph. Klymko et al. \cite{Klymko2012} improved this by providing an embedding algorithm for complete graph $K_{cn+1}$ in a $n\times n$ grid of $K_{c,c}$. In addition, Klymko et al. also proved that any QUBOs which have treewidth bigger than $cn+c$ are not embeddable in a $n\times n$ grid of $K_{c,c}$. Boothy et al. provided a definition of native clique embeddings which generalized the idea of TRIAD \cite{Boothby2016}.

The common point of these approaches is that, they focus on finding an embedding of cliques, which can be induced to embedding of any sub-graphs of the cliques. However, these methods do not take into account of embedding of sparse graphs, although the gap in the number of qubits needed for embedding a clique and its sparse sub-graphs is considerably big. To overcome these problems, Goodrich et al. \cite{Goodrich2018} proposed a biclique virtual hardware framework, which is constructed by compressing the hardware graph. They find a virtual embedding of the logical graph in the virtual hardware framework using the Odd Cycle Traversal (OCT)-based algorithm.

One limitation of virtual embedding is that, not all embeddings in the hardware graph can be interpreted from a virtual embedding in the virtual hardware. As a result, in many cases, methods based on virtual hardware embedding cannot yield optimal or close-optimal solutions. Meanwhile, in theory, bottom-up approach, including heuristic and exact methods, are able to search for solutions in a broader solution space. Bernal et al. expressed minor embedding problem as an IP formulation \cite{Bernal2020}, but their method is limited for small graphs due to large running time of IP. Cai et al. developed a heuristic method \cite{Cai2014} which scales well for sparse graphs by embedding one node at a time. One drawback of this method is that the number of iterations needed to successfully find a feasible embedding which satisfies all three conditions of minor embedding is too large.

In practice, the size of the hardware graph in the latest QPU of Quantum Annealers such as DWave tends to double every 20 months \cite{dwaveQPU}. Thus, the size of embeddable logical graph grows over time. This raises two problems in minor embedding. First, the running time of existing embedding methods may increase unpredictably for large logical graphs. Second, the size of hardware graph can affect the running time and the result of embedding methods. For example, with the same logical graph, the embedding algorithm running on too small hardware graph may lead to an infeasible solution, while the embedding algorithm running on too large hardware may result in large running time. Until now, as far as we know, all approaches solving minor embedding assume that the size of hardware graph is fixed, and they try to find an feasible embedding of the given logical graph which fits to the fixed hardware graph. As a result, if the size of the hardware graph is not chosen appropriately, the performance of the algorithm can suffer. Therefore, to deal with the two problems above, a new embedding method which can provide solutions for large logical graphs in a small running time and adapt the size of the hardware graph along with the expanding of the logical graph is utmost needed.

==> tinhw.tex <==
\begin{enumerate}
    \item Start to read about "adaptive" direction in embedding.
    \item Continue to improve current embedding method with different view.
    \item Try to run proposed QUBO in DWave cloud.
\end{enumerate}
